Drop to Adapt: Learning Discriminative Features for Unsupervised Domain Adaptation

Recent works on domain adaptation exploit adversarial training to obtain domain-invariant feature representations from the joint learning of feature extractor and domain discriminator networks. However, domain adversarial methods render suboptimal performances since they attempt to match the distributions among the domains without considering the task at hand. We propose Drop to Adapt (DTA), which leverages adversarial dropout to learn strongly discriminative features by enforcing the cluster assumption. Accordingly, we design objective functions to support robust domain adaptation. We demonstrate efficacy of the proposed method on various experiments and achieve consistent improvements in both image classification and semantic segmentation tasks. Our source code is available at https://github.com/postBG/DTA.pytorch.

==> analysis.tex <==
\begin{comment}
5. Analysis
5.1. Ablation Study
우리는, 제안한 메소드의 상대적 기여도를 측정하기 위해, VisDA-2017 Classification Dataset에서 Ablation Study를 진행하였다. 여기서 사용한 모델은 Appendix B.1에서 소개한 모델과 같으며, ResNet50과 ResNet101을 사용하여 실험하였다. entmin은 모든 Ablation test에서 사용되었다. 
VAT와 Adversarial Dropout 
먼저 VAT만을 사용한 경우보다, Adversarial Dropout만을 사용한 실험이 모두 더 나은 성능을 보였다. 한편, Adversarial Dropout에 VAT를 함께 사용한 경우, Adversarial Dropout만 사용한 경우보다는 +4%정도, VAT만을 사용한 경우보다는 +8%정도 상승한 것을 확인할 수 있다. 이는 VAT와 Adversarial Dropout이 complementary함을 의미한다. 실제로 []와 Adversarial Dropout [] 에 따르면, 두 메소드가 regularize하는 영역이 서로 다름을 시사하고 있다. 
Channelwise Adversarial Dropout과 Elementwise Adversarial Dropout
Channelwise Adversarial Dropout만을 사용한 모델과 Elementwise Adversarial Dropout만을 사용한 모델을 비교할 경우, Elementwise Adversarial Dropout을 사용한 경우가 더 나은 성능을 보임을 알 수 있다. 하지만, 두가지 Dropout을 함께 사용하는 경우, 하나만 사용한 경우에 비해 더 나은 성능을 보이는 것을 관찰할 수 있는데, 이는 Channelwise Adv Dropout과 Elementwise Adv Dropout이 서로 상호보완적임을 시사한다.

5. Visualizing with Grad-CAM 
우리는 실제로 channel-wise adversarial dropout이 semantic한 정보들을 인코딩하는 channel의 수를 늘리는 데에 효과적인지 확인해보기 위해, channel-wise adversarial dropout을 이용하여 channel을 드랍하기 전과 후 Grad-CAM[]을 비교해보았다. Grad-CAM은 특정 class에 대해 모델이 그 class로 prediction하는데 image의 어느 영역을 보는지 시각화해준다. 우리는 VisDA-2017 Classification에서 학습한 모델들을 이용하여 Grad-CAM을 비교하였으며, Target Dataset에서 모델이 어떻게 행동하는지 비교하였다. 우리는 channel-wise adversarial dropout을 이용하여 ...위치에서 10%의 channel을 드랍하였고, 정답 label에 대한 Grad-CAM을 그려 비교하였다. 결과는 Fig. 2에서 확인할 수 있다.
Fig.2.(a)와 (d)를 비교하면, Source only 모델에서 channel-wise Adversarial Dropout을 적용하면 semantic한 영역들을 많이 잃어버리는 것을 관찰할 수 있다. 반면, 우리의 메소드로 학습한 모델의 경우, 10%의 channel을 드랍하였음에도 불구하고, 여전히 semantic한 정보들을 유지하고 있음을 볼 수 있다.
이러한 결과는 source only model의 경우, 정답 label을 맞추는 경우에도, target feature들이 decision boundary 주위에 위치하고 있음을 시사하기도 한다.
\end{comment}

\subsection{Ablation Studies}\label{ssec:ablation}
\input{tab_ablation}

To analyze the relative importance of \methodname, we conduct comprehensive ablation studies on the VisDA classification dataset. We report results after removing a combination of the three key elements of our method: VAT, element-wise \methodname, and channel-wise \methodname. The entropy loss term is kept constant in all experiments. To emphasize consistency across different model architectures, we experiment on both ResNet-50 and ResNet-101 models. The results can be found in Table~\ref{tab:ablation}. 

\paragraph{VAT and Adversarial Dropout}
We first observe that when each component is used individually, both element-wise and channel-wise \methodname\ are more effective than VAT. Thus, when compared with \methodname\ + VAT, the addition of \methodname\ to VAT is more impactful than when VAT is added to \methodname. Either way, we demonstrate that VAT and \methodname\ strongly complement each other. We reason that the complementary nature of VAT and \methodname\ arise due to the both methods having unique regularization effects on the model; VAT can be seen as a perturbation on the inputs, while \methodname\ acts as a perturbation on the network itself. 

\paragraph{Element-wise and Channel-wise Adversarial Dropout}
We also compare the effectiveness of element-wise and channel-wise \methodname\ when used individually, and observe that element-wise \methodname\ marginally more effective than channel-wise \methodname.  Nevertheless, both can be used simultaneously for stronger adaptation performance.

\subsection{Visualization with Grad-CAM}\label{ssec:gradcam}

To take a closer look at the effects of \methodname, we employ GradCAM [GRADCAM] to highlight the important regions of an image before and after applying \methodname\ to our model. 
